TopSort: A High-Performance Two-Phase Sorting Accelerator Optimized on HBM-based FPGAs

The emergence of high-bandwidth memory (HBM) brings new opportunities to boost the performance of sorting acceleration on FPGAs, which was conventionally bounded by the available off-chip memory bandwidth. However, it is nontrivial for designers to fully utilize this immense bandwidth. First, the existing sorter designs cannot be directly scaled at the increasing rate of available off-chip bandwidth, as the required on-chip resource usage grows at a much faster rate and would bound the sorting performance in turn. Second, designers need an in-depth understanding of HBM characteristics to effectively utilize the HBM bandwidth. To tackle these challenges, we present TopSort, a novel two-phase sorting solution optimized for HBM-based FPGAs. In the first phase, 16 merge trees work in parallel to fully utilize 32 HBM channels. In the second phase, TopSort reuses the logic from phase one to form a wider merge tree to merge the partially sorted results from phase one. TopSort also adopts HBM-specific optimizations to reduce resource overhead and improve bandwidth utilization. TopSort can sort up to 4 GB data using all 32 HBM channels, with an overall sorting performance of 15.6 GB/s. TopSort is 6.7x and 2.2x faster than state-of-the-art CPU and FPGA sorters.

==> Table/existing_hbm_work.tex <==
\begin{table}[!htb]
    \centering
    \caption{Design frequency \& utilized HBM Channels in prior HBM-based FPGA accelerators}
    \label{tab:prior_hbm_work}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccc}
    \hline
    \multicolumn{1}{|c|}{Work} & \multicolumn{1}{c|}{Frequency} & \multicolumn{1}{c|}{Channel Used} & \multicolumn{1}{c|}{Bandwidth Used} \\ \hline
    \multicolumn{1}{|c|}{iccad21} & \multicolumn{1}{c|}{165 MHz} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{247 GB/s} \\ \hline
    \multicolumn{1}{|c|}{sextans} & \multicolumn{1}{c|}{189 MHz} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{289 GB/s} \\ \hline
    \multicolumn{1}{|c|}{sssp} & \multicolumn{1}{c|}{130 MHz} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{200 GB/s} \\ \hline
    \multicolumn{1}{|c|}{spmv} & \multicolumn{1}{c|}{237 MHz} & \multicolumn{1}{c|}{18} & \multicolumn{1}{c|}{258 GB/s} \\ \hline
    \end{tabular}
    }
\end{table}

==> Table/freq.tex <==
\begin{table}[!htb]
    \centering
    \caption{The frequency of the design \zf{swap data in table}}
    \label{tab:design_freq}
    \resizebox{0.7\columnwidth}{!}{
    \begin{tabular}{cc}
    \hline
    \multicolumn{1}{|c|}{Kernel Frequency} & \multicolumn{1}{c|}{HBM Controller Frequency} \\ \hline
    \multicolumn{1}{|c|}{401 MHz} & \multicolumn{1}{c|}{214 MHz} \\ \hline
    \end{tabular}
    }
\end{table}

==> Table/hbm_controller.tex <==
\begin{table}[!htb]
    \centering
    \caption{The resource consumption of a single HBM controller}
    \label{tab:hbm_ctrl_resource}
    \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{ccc}
    \hline
    \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{LUTs Used} & \multicolumn{1}{c|}{Registers Used} \\ \hline
    \multicolumn{1}{|c|}{HBM Controller} & \multicolumn{1}{c|}{5070} & \multicolumn{1}{c|}{6375} \\ \hline
    \end{tabular}
    }
\end{table}

==> Table/model_param.tex <==
\begin{table}[t]
\centering
\caption{Parameters considered in TOP-Sort floorplan}
\begin{tabular}{lrrr}
    \hline
    Symbol & Definition \\
    \hline
    $a_{i}$ & the available resources on $SLR_{i}$ \\
    $u_{i}$ & the number of sub merge trees on $SLR_{i}$ \\
    $L$ & the resources of each sub merge tree \\
    $w$ & the width of an AXI interface \\
    $W$ & the available SSLs \\
    \hline
\end{tabular}
\label{tab:floorplan_model}
\end{table}
